Stochastic Proximal Gradient Algorithm with Minibatches. Application to Large Scale Learning Models

Stochastic optimization lies at the core of most statistical learning models. The recent great development of stochastic algorithmic tools focused significantly onto proximal gradient iterations, in order to find an efficient approach for nonsmooth (composite) population risk functions. The complexity of finding optimal predictors by minimizing regularized risk is largely understood for simple regularizations such as $\ell_1/\ell_2$ norms. However, more complex properties desired for the predictor necessitates highly difficult regularizers as used in grouped lasso or graph trend filtering. In this chapter we develop and analyze minibatch variants of stochastic proximal gradient algorithm for general composite objective functions with stochastic nonsmooth components. We provide iteration complexity for constant and variable stepsize policies obtaining that, for minibatch size $N$, after $\mathcal{O}(\frac{1}{N\epsilon})$ iterations $\epsilon-$suboptimality is attained in expected quadratic distance to optimal solution. The numerical tests on $\ell_2-$regularized SVMs and parametric sparse representation problems confirm the theoretical behaviour and surpasses minibatch SGD performance.

==> Stochastic proximal gradient algorithm with minibatches/parametric.tex <==
% Our model is:

% \begin{align*}
% 	\min\limits_x \;\; \frac{1}{2m}\|Tx-y\|^2_2 + +
% 	\frac{\alpha}{2} \|x\|^2_2 + 
% 	\frac{\lambda}{p}\|\Delta x\|_1.
% \end{align*}
% where $T \in \rset^{m \times n}, \Delta \in \rset^{p \times n}$.
% Good settings are the following:
% \begin{itemize}
% 	\item[1.] $m >> n, p >>n, \alpha \ge 0$
% 	\item[2.] $m < n, p>>n, \alpha>0$
% \end{itemize}

Given signal $y \in \rset^m$
and
overcomplete dictionary $T \in \rset^{m \times n}$
(whose columns are also called atoms),
sparse representation~\cite{Ela:10}
aims to find the sparse signal $x\in\rset^n$
by projecting $y$ to a much smaller subspace
generated by a subset of the columns from $T$.
Sparse representation is a key ingredient in dictionary learning techniques~\cite{DumIro:18}
and here we focus on the multi-parametric sparse representation model proposed in \cite{StoIro:19}.
Note that this was analyzed in the past in non-minibatch SPG form~\cite{PatIro:20} which we denote with SSPG in the following.
The multi-parametric representation problem is given by:
%-------------------
\be
\begin{aligned}
	& \underset{x}{\min}
	& & \|Tx-y\|^2_2 \\
	& \text{s.t.}
	& & \|\Delta x\|_1 \le \delta,
\end{aligned}
\label{eq:optprob}
\ee
%-------------------
where $T$ and $x$ correspond to the dictionary and, respectively, the resulting sparse representation,
with sparsity being imposed on a scaled subspace $\Delta x$ with $\Delta\in\rset^{p\times n}$.
In pursuit of \eref{problem_intro},
we move to the exact penalty problem $\min_x \frac{1}{2m}\norm{Tx - y}^2_2 + \lambda \norm{\Delta x }_1$. In order to limit the solution norm we further regularize the unconstrained objective using an $\ell_2$ term as follows:
%-------------------
\begin{align*}
	\min\limits_x \;\; \frac{1}{2m}\|Tx-y\|^2_2 +
	\frac{\alpha}{2} \|x\|^2_2 + 
	\frac{\lambda}{p}\|\Delta x\|_1.
\end{align*}
\label{eq:strongprob}
%-------------------
The decomposition which puts the above formulation into model \eqref{problem_intro} consists of:
\be
f(x;\xi) = \frac{1}{2} (T_\xi x-y_\xi)^2_2 + 
\frac{\alpha}{2} \|x\|^2_2
\label{eq:sp_smooth}
\ee
where $T_\xi$ represents line $\xi$ of matrix $T$, and 
\be
h(x; \xi) = \lambda |\Delta_\xi x|.
\label{eq:sp_nonsmooth}
\ee
To compute the SPG-M iteration for the sparse representation problem, we note that 
\begin{align*}
	\text{prox}_{h,\mu}(x;\I) 
	& = \arg\min_z \; \frac{\lambda}{N}\norm{\Delta_I z}_1 + \frac{1}{2\mu}\norm{z-x}^2.
\end{align*}
Equivalently, once we find dual vector
\begin{align*}
	z^{k}  & = \arg\min_{-1 \le z \le 1}  \frac{\mu\lambda^2}{2N^2} \norm{\Delta_I^Tz}^2 - \frac{\lambda}{N}z^T\Delta_I t 
\end{align*}
then we can easily compute $\text{prox}_{h,\mu}(x;I) = x - \frac{\mu \lambda}{N} \Delta_I^T z$.
We are ready to formulate the resulting particular variant of SPG-M.
\begin{flushleft}
	\textbf{SPG-M - Sparse Representation  (SPGM-SR)}: 
	\quad For $k\geq 0$ compute \\
	1. Choose randomly i.i.d. $N-$tuple $I^k \subset \Omega$ \\
	2. Update: 
	\begin{align*}
	y^{k}  & =  \left[ I_n - \frac{\mu_k}{N} \left(T_{I_k}^T T_{I_k} + N\alpha I_n \right)\right] x^k + \frac{\mu_k}{N} T_{I_k}^T y_{I_k}\\
	z^{k}  & = \arg\min_{-1 \le z \le 1}  \frac{\mu\lambda^2}{2N^2} \norm{\Delta_I^Tz}^2 - \frac{\lambda}{N}z^T\Delta_I t \\
	x^{k+1} & = y^k - \frac{\mu_k\lambda}{N} \Delta_I^T z^k
	\end{align*}
	3. If the stoppping criterion holds, then \textbf{STOP}, otherwise $k = k+1$.
\end{flushleft}
% %---------------------------
% \pdffig{spgm-gensr-linstep2}
%   {SPG-M with Variable stepsize ($\alpha=0.2$)}
%   {fig:spgm-gensr-linstep2}
% %---------------------------
% %---------------------------
% \pdffig{spgm-gensr-mixedstep2}
%   {SPG-M with Mixed stepsize ($\alpha=0.2$)}
%   {fig:spgm-gensr-mixedstep2}
% %---------------------------

%---------------------------
\begin{figure}[t]
    \centering
    \begin{minipage}{0.5\textwidth}
	\centering
	\includegraphics[width=\textwidth]{spgm-gensr-linstep2}
	\caption{Variable stepsize ($\alpha=0.2$)}
	\label{fig:spgm-gensr-linstep2}
	\end{minipage}\hfill
	\begin{minipage}{0.5\textwidth}
	\centering
	\includegraphics[width=\textwidth]{spgm-gensr-mixedstep2}
	\caption{Mixed stepsize ($\alpha=0.2$)}
	\label{fig:spgm-gensr-mixedstep2}
	\end{minipage}
\end{figure}
%---------------------------
%---------------------------
\begin{figure}[t]
    \centering
    \begin{minipage}{0.5\textwidth}
	\centering
	\includegraphics[width=\textwidth]{spgm-gensr-linstep3}
	\caption{Variable stepsize ($\alpha=0.7$)}
	\label{fig:spgm-gensr-linstep3}
	\end{minipage}\hfill
	\begin{minipage}{0.5\textwidth}
	\centering
	\includegraphics[width=\textwidth]{spgm-gensr-mixedstep3}
	\caption{Mixed stepsize ($\alpha=0.7$)}
	\label{fig:spgm-gensr-mixedstep3}
	\end{minipage}
\end{figure}
%---------------------------

We proceed with numerical experiments that depict
SPG-M with various batch sizes $N$
and compare them with SSPG~\cite{PatIro:20},
which is equivalent to SPG-M where $N=1$.
In our experiments we use batches of $N=\{1, 10, 50, 100\}$ samples
from a population of $m=400$
using dictionaries with $n=200$ atoms.
We fix $\lambda=5\dot 10^{-4}$ and stop the algorithms
when the euclidean distance between current solution $x$ 
and the optimum $x^{\star}$ is less than $\varepsilon=10^{-3}$.
CVX is used to determine $x^\star$ within a $\varepsilon=10^{-6}$ margin.

%Past experiments~\cite{PatIro:20} indicated that larger values of $\alpha$ lead to a slow-down in convergence.
Here we choose two scenarios:
one where $\alpha=0.2$ and all methods provide adequate performance,
depicted in Figures \ref{fig:spgm-gensr-linstep2} and \ref{fig:spgm-gensr-mixedstep2},
and a second where $\alpha=0.7$ is larger and stomps performance as can be seen in the first ten iterations
of Figures \ref{fig:spgm-gensr-linstep3} and \ref{fig:spgm-gensr-mixedstep3}.
In these figures we can also observe that the mixed stepsize indeed provides much better convergence rate and that the multibatch algorithm is always ahead of the single batch SSPG version. 
% n_nonzero_coefs = 3     # sparsity (s)
% n_samples = 1           # number of signals (N)
% alpha = 0.7    # l2 weight
% lam = .0005     # l1 weight
% eps = 1e-3      # precision
% batchSizesToTry = [10, 50, 100]
% n_features = n_components * 2

We continue our investigation by adapting the minibatch stochastic gradient descent method to the parametric sparse representation problem which leads to the following algorithm:

\begin{flushleft}
	\textbf{SGD-M - Sparse Representation  (SGDM-SR)}:
	\quad For $k\geq 0$ compute \\
	1. Choose randomly i.i.d. $N-$tuple $I^k \subset \Omega$ \\
	2. Update: 
	\begin{align*}
	x^{k+1} & = x^k - \frac{\mu_k}{N} \left(T_{I_k}^T T_{I_k} + N\alpha I_n \right) x^k + \frac{\mu_k}{N} T_{I_k}^T y_{I_k} - \frac{\mu_k\lambda}{N} \sum\limits_{i \in I^k} \text{sgn}(\Delta_i x^k) \Delta_i^T,
	\end{align*}
	where $\text{sgn}(\Delta_i x) = \begin{cases} +1, & \Delta_i x > 0 \\ -1, & \Delta_i x< 0 \\ 0, & \Delta_i x = 0\end{cases}$
	
	3. If the stoppping criterion holds, then \textbf{STOP}, otherwise $k = k+1$.
\end{flushleft}

When applying SGDM-SR on the same initial data as our experiment with $\alpha=0.7$ with the same parametrization and batch sizes we obtain the results depicted in Figure~\ref{fig:spgm-gensr-sgd}.
Here the non-minibatch version of SGD is clearly less performant than SPG-M,
but what is most interesting is that the minibatch version
for all batch sizes behaves identically and
takes 100 iterations to recover and reach the optimum around iteration 150.
% %---------------------------
% \pdffig{spgm-gensr-linstep3}
%   {SPG-M with Variable stepsize ($\alpha=0.7$)}
%   {fig:spgm-gensr-linstep3}
% %---------------------------
% %---------------------------
% \pdffig{spgm-gensr-mixedstep3}
%   {SPG-M with Mixed stepsize ($\alpha=0.7$)}
%   {fig:spgm-gensr-mixedstep3}
% %---------------------------
%---------------------------
\pdffig{spgm-gensr-linstep-sgd}
  {SPG-M and SGD with Variable stepsize. The other batch sizes were identical with N=100 for SGD. ($\alpha=0.7$)}
  {fig:spgm-gensr-sgd}
%---------------------------
